Quantum trapdoor functions from classical one-way functions

We formalize and study the notion of a quantum trapdoor function. This is an efficiently computable unitary that takes as input a "public" quantum state and a classical string $x$, and outputs a quantum state. This map is such that (i) it is hard to invert, in the sense that it is hard to recover $x$ given the output state (and many copies of the public state), and (ii) there is a classical trapdoor that allows efficient inversion. We show that a quantum trapdoor function can be constructed from any quantum-secure one-way function. A direct consequence of this result is that, assuming just the existence of quantum-secure one-way functions, there exists a public-key encryption scheme with a (pure) quantum public key.

==> commands.tex <==
\newcommand{\etal}{{et al. }}
\usepackage{amsfonts,latexsym,graphicx,amssymb,amsmath,enumitem,physics}
\usepackage{amsthm}
\usepackage{fullpage}
\usepackage{color} % for textcolor
\usepackage{hyperref,cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% General %%%%%%%%%%%%%%%%%%%%%%%%%
\mathchardef\mhyphen="2D
\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\bit}{\{0,1\}}
\newcommand{\seclam}{1^\lambda}
\newcommand{\msk}{\mathsf{msk}}
\newcommand{\key}{\mathsf{key}}
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\vk}{\mathsf{vk}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\ct}{\mathsf{ct}}
\newcommand{\negl}{\mathsf{negl}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\BQP}{\mathsf{BQP}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\from}{\gets}
\newcommand{\prg}{\mathsf{PRG}}
\newcommand{\Rq}{R_q}
\newcommand{\Zq}{\Z_q}
\newcommand{\st}{^*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Sets, brackets shorthand %%%%%%%%%%%%%
\newcommand{\scl}[1]{\set{{#1}_\lambda}_{\lambda \in \N}}
\newcommand{\sck}[1]{\set{{#1}_\kappa}_{\kappa \in \N}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sset}[1]{\{#1\}}
\newcommand{\brackets}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\Brackets}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\nat}[1]{\ensuremath{\Brackets{1, #1}}}
\newcommand{\natz}[1]{\ensuremath{\set{0, 1, \ldots, #1}}}
\newcommand{\nato}[2]{\ensuremath{\set{#1, \ldots, #2}}}
% \newcommand{\ket}[1]{|#1\rangle}
% \newcommand{\bra}[1]{\langle#1|}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% Calligraphic letters %%%%%%%%%%%%%%%%%
%%% Missing letters F, H, L, N, O, P, Z
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\E}{\ensuremath{\mathcal{E}}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\renewcommand{\P}{\ensuremath{\mathcal{P}}}
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\U}{\ensuremath{\mathcal{U}}}
\newcommand{\V}{\ensuremath{\mathcal{V}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}
\newcommand{\X}{\ensuremath{\mathcal{X}}}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}}
\newcommand{\mat}[1]{\mathbf{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% Theorem, lemma, etc %%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{claim}{Claim}[theorem]
\newtheorem{fact}{Fact}[theorem]
\newtheorem{definition}{Definition}[theorem]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}[theorem]
\newtheorem{remark}{Remark}[theorem]
\newtheorem{construction}{Construction}
%\newtheorem{cclaim}{Claim}
% keep the following for lncs
\newtheorem{assumption}{Assumption}
\newtheorem{observation}{Observation}

%%%%%%%%%%% Referring to stuff %%%%%%%%%%% %%%%%%%%%%%%%%
\newcommand{\defref}[1]{Definition~\protect\ref{def:#1}}
\newcommand{\secref}[1]{Section~\protect\ref{sec:#1}}
\newcommand{\appref}[1]{Appendix~\protect\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\protect\ref{fig:#1}}
\newcommand{\tblref}[1]{Table~\protect\ref{tbl:#1}}
\newcommand{\tableref}[1]{Table~\protect\ref{table:#1}}

\newcommand{\thmref}[1]{Theorem~\protect\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\protect\ref{lem:#1}}
\newcommand{\obsref}[1]{Observation~\protect\ref{obs:#1}}
\newcommand{\clmref}[1]{Claim~\protect\ref{clm:#1}}
\newcommand{\claimref}[1]{Claim~\protect\ref{claim:#1}}
\newcommand{\assref}[1]{Assumption~\protect\ref{ass:#1}}

\newcommand{\corref}[1]{Corollary~\protect\ref{cor:#1}}
\newcommand{\fctref}[1]{Fact~\protect\ref{fct:#1}}
\newcommand{\eqnref}[1]{Equation~(\protect\ref{eqn:#1})}
\newcommand{\rmkref}[1]{Remark~\protect\ref{rmk:#1}}
\newcommand{\asmref}[1]{Assumption~\protect\ref{asm:#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Protocols, figures %%%%%%%%%%
\renewcommand{\figurename}{Protocol}

\newlength{\protowidth}
\newcommand{\pprotocol}[5]{
{\begin{figure*}[#4]
\begin{center}
\setlength{\protowidth}{\textwidth}

%\addtolength{\protowidth}{-3\intextsep}

% \fbox{
%         \small
%         \hbox{\quad
%         \begin{minipage}{\protowidth}
%         \begin{center}
%         {\bf #1}
%         \end{center}
%         #5
%         \end{minipage}
%         \quad}
%         }
        {
        \hrulefill \vspace{5pt}
        \small
        {\quad
        \begin{minipage}{\protowidth}
        \begin{center}
        {\bf #1}
        \end{center}
        #5

        \hrulefill

        \end{minipage}
        \quad}
        }

        \caption{\label{#3} #2}
\end{center}
\vspace{-4ex}
\end{figure*}
} }


\newcommand{\protocol}[4]{
\pprotocol{#1}{#2}{#3}{tbh!}{#4} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%% prelims %%%%%%%%%%
\newcommand{\rlweqchi}{\mathsf{RLWE}_{R, q,\chi}}
\newcommand{\Rn}{R_n}
\newcommand{\Rnqn}{R_{n, q_n}}
\newcommand{\Rnq}{R_{n,q}}
\newcommand{\Rqn}{R_{n,q}}
\newcommand{\gentrap}{\textsc{GenTrap}}
\newcommand{\inv}{\textsc{Invert}}
\newcommand{\rhoXE}{\rho_{XE}}
\newcommand{\rhoxE}{\rho^x_E}
\newcommand{\pguess}{p_{\mathrm{guess}}}
\newcommand{\minent}{{H_{\infty}}}
\newcommand{\dm}{\mathsf{D}}
\newcommand{\dg}{\dagger}
\newcommand{\Id}{\mathsf{Id}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% NTCFs %%%%%%%%%%
\newcommand{\trap}{\tau}
\newcommand{\trapf}{\kappa}
\newcommand{\supp}{\textsc{Supp}}
\newcommand{\genf}{\textsc{Gen}_{\mathcal{F}}}
\newcommand{\invf}{\textsc{Inv}_{\mathcal{F}}}
\newcommand{\chkf}{\textsc{Chk}_{\mathcal{F}}}
\newcommand{\sampf}{\textsc{Samp}_{\mathcal{F}}}
\newcommand{\J}{\mathsf{BitDecomp}}
\newcommand{\bdx}{\overline{x}}
\newcommand{\hatg}[1]{\hat{G}_{{#1}}}
\newcommand{\Es}[1]{E_{#1}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mata}{\vec{a}}
\newcommand{\mate}{\vec{e}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Quantum supremacy %%%%%%%%%%
\newcommand{\cnt}{\mathsf{count}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% randomness %%%%%%%%%%
\newcommand{\hash}{H}
\newcommand{\PHkymd}{\mathsf{P}_{k,\hash}^{y,m,d}}
\newcommand{\BHky}{\mathsf{B}_{k,\hash}^y}
\newcommand{\phist}{\phi}
\newcommand{\stateone}{\rho}
\newcommand{\comp}[1]{\overline{#1}}
\newcommand{\My}{M_y}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\phione}{\phi_1}
\newcommand{\phitwo}{\phi_2}
\newcommand{\acchk}{\mathsf{Acc}_{\hash,k}}
\newcommand{\prbd}{q}
\newcommand{\query}{Q}
\newcommand{\HfourQ}{\calH_{4 \query}}
\newcommand{\Axh}{\mathsf{A}_{\hash}^{x_0, x_1, h}}
\newcommand{\Bxh}{\mathsf{B}_{\hash}^{x_0, x_1, h}}
\newcommand{\RH}{\R_{\hash}}
